Internet of Agents: Weaving a Web of Heterogeneous Agents for Collaborative Intelligence

The rapid advancement of large language models (LLMs) has paved the way for the development of highly capable autonomous agents. However, existing multi-agent frameworks often struggle with integrating diverse capable third-party agents due to reliance on agents defined within their own ecosystems. They also face challenges in simulating distributed environments, as most frameworks are limited to single-device setups. Furthermore, these frameworks often rely on hard-coded communication pipelines, limiting their adaptability to dynamic task requirements. Inspired by the concept of the Internet, we propose the Internet of Agents (IoA), a novel framework that addresses these limitations by providing a flexible and scalable platform for LLM-based multi-agent collaboration. IoA introduces an agent integration protocol, an instant-messaging-like architecture design, and dynamic mechanisms for agent teaming and conversation flow control. Through extensive experiments on general assistant tasks, embodied AI tasks, and retrieval-augmented generation benchmarks, we demonstrate that IoA consistently outperforms state-of-the-art baselines, showcasing its ability to facilitate effective collaboration among heterogeneous agents. IoA represents a step towards linking diverse agents in an Internet-like environment, where agents can seamlessly collaborate to achieve greater intelligence and capabilities. Our codebase has been released at \url{https://github.com/OpenBMB/IoA}.

==> figs_code/team_up.tex <==
\begin{wrapfigure}{r}{0.53\textwidth}
    \centering
    \vspace{-1.5em}
    % \vspace{-1.2em}
    \includegraphics[width=0.5\textwidth]{figs/team_formation_precision.pdf}
    \vspace{-1em}
    \caption{Top@k of recall rate between \textit{Regular} and \textit{Nested}}
    \label{fig:Top@k-recall-rate}
\end{wrapfigure}



==> sections/framework.tex <==
% \section{Framework Design of \framework}
% \label{sec:framework}
% \input{figs_code/layers}
% In this section, we present a feasible framework design of \framework. To facilitate effective collaboration among autonomous agents, an IM application specifically designed for agents should include two major components: the client and the server. The server is responsible for message forwarding, group chat maintenance, agent registry maintenance, etc. It should be capable of hosting connections between distributed agents, allowing agents running on different devices and with varying capabilities to register, discover each other, and initiate group chats. The client, on the other hand, acts as a wrapper for different agents, many of which are not inherently designed for communication. The client provides the necessary communication functionalities through an adapter that aligns each agent with the specified protocol. For agents not designed for communication, an additional LLM within the client handles communication among agents. Agents that can communicate by design can adhere to the message protocol defined by the IM app to integrate seamlessly.

% The architecture of both the client and server in an agent IM app can be structured into three layers. From top to bottom are: \textit{Interaction Layer, Data Layer}, and \textit{Foundation Layer}, as shown in~\cref{fig:layer-architecture}. Each layer has specific responsibilities that contribute to the overall functionality and efficiency of the system. Additionally, the message protocol between the client and the server plays a crucial role in defining the communication and collaboration mechanisms among agents, as it specifies the types of information that can be transmitted and shared.

% \textbf{Interaction Layer.}
% The Interaction Layer facilitates effective communication and collaboration between agents. It ensures that agents can interact seamlessly, respond to ongoing tasks, and form teams as needed. 

% \textbf{Data Layer.}
% The Data Layer manages information related to agents, group chats, and tasks. This layer organizes and maintains the data that agents need to collaborate effectively within the IM app environment.

% \textbf{Foundation Layer.}
% The Foundation Layer provides the essential infrastructure necessary for agent integration, data management, and network communication. This layer ensures seamless integration of agents into the system and should provide robust data and network services to support their operations.

% \subsection{Client}
% The client side of an agent IM app employs a layered architecture to integrate and manage diverse agents, ensuring they can collaborate and communicate effectively.

% At the Interaction Layer, the client facilitates dynamic communication and team formation. The Team Formation Block is designed to identify suitable collaborators for incoming tasks, streamlining the process of forming effective teams. Meanwhile, the Communication Block manages all ongoing group chats related to the current agent, ensuring timely and relevant responses.

% The Data Layer of the client is dedicated to handling critical information about agents, group chats, and tasks. Within this layer, the Agent Contact Block functions like a contact list, storing details about previously connected agents and any pertinent notes from past interactions. This information is invaluable for future collaborations. The Group Info Block keeps detailed records of group chats, including histories, member details, and objectives. Concurrently, the Task Management Block tracks the status of all tasks within these group chats, providing agents with the necessary insights to monitor progress and make informed decisions.

% At the Foundation Layer, the client ensures robust infrastructure for agent integration and data services. The Agent Integration Block outlines the protocols and interfaces required for seamless agent integration, such as \texttt{\textbf{run}(task\_desc) $\rightarrow$ task\_id} for task execution and \texttt{\textbf{read\_memory}(task\_id) $\rightarrow$ history} for retrieving task-related memory. Additionally, the Data Infra Block supports data persistence, retrieval, and access control. Complementing these, the Network Infra Block manages the communication between the client and the server, ensuring reliable and efficient data transmission.

% \subsection{Server}
% The server side of an agent IM app manages the overall infrastructure, facilitating agent discovery, group setup, and efficient message routing, while maintaining robust data and network services.

% In the Interaction Layer, the server enables agents to discover each other, initiate group chats, and communicate seamlessly. The Agent Query Block allows agents to search for others based on specific characteristics, aiding effective team formation. The Group Setup Block streamlines the creation of group chats by allowing agents to specify desired teammates. Meanwhile, the Message Routing Block ensures that messages from agents within different group chats are correctly forwarded to the appropriate members, maintaining a smooth flow of communication.

% The Data Layer of the server focuses on supporting efficient agent queries and group communications. The Agent Registry Block stores detailed information about agents, including their accessible tools, average costs, and capability descriptions. This registry is crucial for the Agent Query Block to find suitable agents. The Session Management Block maintains active connection sessions between the server and client agents, ensuring that messages can be routed reliably, supporting continuous communication.

% At the Foundation Layer, the server provides essential infrastructure for data management, network communication, and security. Similar to the client, it includes the Data Infra Block and the Network Infra Block, which handle data persistence, retrieval, and reliable network communication between the server and clients. Additionally, the Security Block plays a critical role in authentication and authorization, ensuring that only authorized agents can connect to the server and participate in communications, thereby maintaining the integrity and security of the agent IM app.

\section{Framework Design of \framework}
\label{sec:framework}
\input{figs_code/layers}
In this section, we present the instant-messaging-app-like framework design of \framework, which aims to facilitate effective collaboration among autonomous agents. The framework consists of two main components: server and client. The server is responsible for agent registration, discovery, and message routing, enabling agents running on different devices and with varying capabilities to find each other and communicate. The client acts as a wrapper for different agents, providing the necessary communication functionalities and adapting them to the specified protocol. For agents not designed for communication, an additional LLM within the client handles the communication among agents.

The architecture of both the client and server in \framework can be structured into three layers: \textit{Interaction Layer}, \textit{Data Layer}, and \textit{Foundation Layer}, as shown in~\cref{fig:layer-architecture}. Each layer has specific responsibilities that contribute to the overall functionality and efficiency of the system. The message protocol between the client and the server plays a crucial role in defining the communication and collaboration mechanisms among agents, enabling information transmission and conversational state switch.

\textbf{Interaction Layer.}
The Interaction Layer facilitates seamless communication and collaboration between agents, enabling them to interact, respond to ongoing tasks, and form teams as needed.

\textbf{Data Layer.}
The Data Layer manages information related to agents, group chats, and tasks, organizing and maintaining the data that agents need to collaborate effectively within the framework.

\textbf{Foundation Layer.}
The Foundation Layer provides the essential infrastructure for agent integration, data management, and network communication, ensuring seamless integration of agents into the system and providing robust data and network services to support their operations.

\subsection{Client}
The client side of \framework integrate and manage diverse agents, ensuring they can collaborate and communicate effectively.

At the Interaction Layer, the client facilitates dynamic communication and team formation. The Team Formation Block identifies suitable collaborators for incoming tasks, streamlining the process of forming effective teams. The Communication Block manages all ongoing group chats related to the current agent, ensuring timely and relevant responses.

The Data Layer of the client handles critical information about agents, group chats, and tasks. The Agent Contact Block functions like a contact list, storing details about previously connected agents and pertinent notes from past interactions. The Group Info Block keeps detailed records of group chats, including histories, member details, and objectives. The Task Management Block tracks the status of all tasks within these group chats, providing agents with the necessary insights to monitor progress and make informed decisions.

At the Foundation Layer, the client ensures robust infrastructure for agent integration and data services. The Agent Integration Block outlines the protocols and interfaces required for seamless integration of third-party agents, such as \texttt{\textbf{run}(task\_desc) $\rightarrow$ task\_id} for task execution and \texttt{\textbf{read\_memory}(task\_id) $\rightarrow$ history} for retrieving task-related memory. The Data Infra Block supports data persistence, retrieval, and access control, while the Network Infra Block manages the communication between the client and the server, ensuring reliable and efficient data transmission.

\subsection{Server}
The server side of \framework manages the overall infrastructure, facilitating agent discovery, group setup, and efficient message routing, while maintaining robust data and network services.

In the Interaction Layer, the server enables agents to discover each other, initiate group chats, and communicate seamlessly. The Agent Query Block allows agents to search for others based on specific characteristics, aiding effective team formation. The Group Setup Block streamlines the creation of group chats by allowing agents to specify desired teammates. The Message Routing Block ensures that messages from agents within different group chats are correctly forwarded to the appropriate members, maintaining a smooth flow of communication.

The Data Layer of the server supports efficient agent queries and group communications. The Agent Registry Block stores detailed information about agents, including their accessible tools, average costs, and capability descriptions, which is crucial for the Agent Query Block to find suitable agents. The Session Management Block maintains active connection sessions between the server and client agents, ensuring that messages can be routed reliably, supporting continuous communication.

At the Foundation Layer, the server provides essential infrastructure for data management, network communication, and security. The Data Infra Block and the Network Infra Block handle data persistence, retrieval, and reliable network communication between the server and clients. The Security Block plays a critical role in authentication and authorization, ensuring that only authorized agents can connect to the server and participate in communications, maintaining the integrity and security of the framework.

==> sections/prototype.tex <==
\section{Key Mechanisms in \framework}
\label{sec:prototype}

In this section, we introduce the key mechanisms implemented in \framework. \framework is built upon the conceptual design presented in~\cref{sec:framework} and incorporates several key features that enable effective collaboration among agents with diverse capabilities. These features include Autonomous Nested Team Formation, Autonomous Conversation Flow Control, and Comprehensive Message Protocol Design. \framework aims to facilitate the dynamic formation of agent teams and streamline communication processes, ultimately enhancing the collective problem-solving capabilities of multi-agent systems.

\subsection{Autonomous Nested Team Formation}
\label{sec:prototype-team-formation}

% The primary motivation behind the autonomous nested team formation mechanism is to enable scalable and flexible task execution. Traditional multi-agent systems often struggle with static team compositions and limited scalability. By allowing agents to autonomously form nested teams, \framework can dynamically adjust to the complexity and scope of the task at hand. This mechanism ensures that agents with the appropriate skills and resources are engaged, leading to more efficient and effective problem-solving.

% \paragraph{Mechanism Overview}

% Autonomous nested team formation allows agents to dynamically form and expand teams to tackle complex tasks efficiently. This mechanism leverages the server's capabilities to discover and connect agents based on their skills and characteristics, facilitating scalable task execution in a multi-agent system.

% Let $\mathcal{C}$ denote the set of all clients in the system, and let $\mathcal{T}$ denote the task space. For each client $c_i \in \mathcal{C}$, we require it to provide a description $d_i$ of the integrated agent's skills and capabilities.

% When a task $t \in \mathcal{T}$ is assigned to a client $c_i$, it enters the "team formation" phase, where it has access to two essential tools: $\texttt{search\_agent}$ and $\texttt{launch\_group\_chat}$. The $\texttt{search\_agent}$ tool allows the client to discover other agents with specific characteristics by querying the server's Agent Registry. The parameter for this tool is a list of desired characteristics $\mathcal{L}_d = [l_1, l_2, \dots, l_k]$, which are freely generated by the client and not limited to a pre-defined set. The $\texttt{search\_agent}$ tool returns a subset of clients $\mathcal{C}_d \subseteq \mathcal{C}$ such that for each $c_j \in \mathcal{C}_d$, the description $d_j$ is semantically similar to the desired characteristics in $\mathcal{L}_d$.

% The $\texttt{launch\_group\_chat}$ tool enables the client to initiate a group chat with the selected agents. Let $\mathcal{G}$ denote the set of all group chats, and let $g_l \in \mathcal{G}$ be a specific group chat. Each group chat $g_l$ is associated with a set of participating clients $\mathcal{C}_l \subseteq \mathcal{C}$ and a task $t_l \in \mathcal{T}$.

% The LLM in the client is responsible for deciding which tool to call during the team formation phase. It takes into account the retrieved information from the server, local information from the Agent Contact Block, and the task requirements to determine the most suitable agents for collaboration. Mathematically, the LLM's decision-making process can be modeled as a function $f: \mathcal{P}(\mathcal{C}) \times \mathcal{T} \to \{\texttt{search\_agent}, \texttt{launch\_group\_chat}\}$, where $\mathcal{P}(\cdot)$ denotes the power set. The function $f$ takes as input the set of discovered clients $\mathcal{C}_d$ and the task $t$, and returns the appropriate tool to be called.

% By formalizing the autonomous nested team formation mechanism using mathematical language, we can better understand the underlying processes and decision-making involved in dynamically forming and expanding teams. This formalization also provides a foundation for further analysis and optimization of the mechanism, enabling the development of more efficient and effective multi-agent collaboration strategies.





% The primary motivation behind the autonomous nested team formation mechanism is to enable scalable and flexible task execution. Traditional multi-agent systems often struggle with static team compositions and limited scalability. By allowing agents to autonomously form nested teams, \framework can dynamically adjust to the complexity and scope of the task at hand. This mechanism ensures that agents with the appropriate skills and resources are engaged, leading to more efficient and effective problem-solving.

% \paragraph{Mechanism Overview}

% Autonomous nested team formation allows clients to dynamically form and expand teams to tackle complex tasks efficiently. This mechanism leverages the server's capabilities to discover and connect clients based on their skills and characteristics, facilitating scalable task execution in a multi-agent system.

% Let $\mathcal{C}$ denote the set of all clients in the system. For each client $a_i \in \mathcal{A}$, we require it to provide a description $d_i$ of the integrated agent's skills and capabilities when it is registered to the server. 
% When a task $t$ is assigned to a client $c_i$, it enters the Team Formation Block, where it has access to two essential tools: $\texttt{search\_client}$ and $\texttt{launch\_group\_chat}$. The $\texttt{search\_client}$ tool allows the client to discover other clients with specific characteristics by querying the server's Agent Registry. It accepts a list of desired characteristics $\mathcal{L}_d = [l_1, l_2, \dots, l_k]$ freely generated by the client based on $t$. The $\texttt{search\_client}$ tool returns a subset of clients $\mathcal{C}_d \subseteq \mathcal{C}$ such that for each $c_j \in \mathcal{C}_d$, the description $d_j$ is semantically similar to the desired characteristics in $\mathcal{L}_d$. The $\texttt{launch\_group\_chat}$ tool enables the client to initiate a group chat with the selected clients. The LLM in the client is responsible for deciding which tool to call during the team formation phase. It takes into account the retrieved information from the server, local information from its Agent Contact Block, and the task to determine the most suitable clients for collaboration. Mathematically, the LLM's decision-making process can be modeled as a function $f: \mathcal{P}(\mathcal{C}) \times \mathcal{T} \to \{\texttt{search\_client}, \texttt{launch\_group\_chat}\}$, where $\mathcal{P}(\cdot)$ denotes the power set. The function $f$ takes as input the set of discovered clients $\mathcal{C}_d$ and the task $t$, and returns the appropriate tool to be called.

% \paragraph{Nested Team Formation}
% \input{figs_code/nested-teamup}
% However, in some cases, a single group may not be sufficient to complete a task perfectly. During discussions, agents may realize that they require assistance from other agents with specific expertise. To address this, \framework supports nested team formation, allowing agents to initiate sub-group chats for sub-tasks. \cref{fig:nested-teamup} presents a simple example.

% Let $t_l$ be a sub-task assigned to client $c_i\in\mathcal{C}$ in group chat $g$, if $c_i$ determines that it cannot complete the task alone, it can again search for proper clients for $t_l$ and initiate a new sub-group chat $g_{l}$ and invite a subset of other agents $\mathcal{C}_{l} \subseteq \mathcal{C}$ to collaborate on the specific sub-task. This process can continue recursively, forming a tree-like structure where the root represents the initial overall goal's group chat, and the branches represent the group chats for different sub-tasks. 

% Furthermore, the nested team formation mechanism helps to manage the complexity of communication within large agent teams. By organizing the collaboration into a hierarchical structure of group chats, each focusing on a specific sub-task, the communication overhead is reduced, and the conversation flow becomes more manageable. Let By decomposing a task into sub-tasks and allocating them to sub-group chats, the total edges of the communication graph can be reduced from $|\mathcal{C}_l|(|\mathcal{C}_l|-1)$ to $\sum_{j} |\mathcal{C}_{lj}|$, where $\mathcal{C}_{lj}$ represents the set of messages exchanged within the sub-group chat $g_{lj}$. This reduction in communication complexity leads to more efficient and focused collaboration among agents.

% Let $g_l \in \mathcal{G}$ be a group chat assigned with a task $t_l \in \mathcal{T}$. During the discussion, an client $c_i \in \mathcal{C}_l$ may be assigned a sub-task $s_{lj} \in \mathcal{S}_l$, where $\mathcal{S}_l$ represents the set of sub-tasks decomposed from $t_l$. If the client $c_i$ determines that it cannot complete the sub-task $s_{lj}$ alone, it can again search for clients with the required skills and expertise and initiate a new sub-group chat $g_{lj}$ and invite relevant clients to collaborate on the sub-task $s_{lj}$. This process can continue recursively, forming a tree-like structure where the root represents the initial overall goal's group chat, and the branches represent the group chats for different sub-tasks, denoted by $h(g_l, s_{lj}) = g_{lj}$, where $s_{lj} \in \mathcal{S}_l$.

% Furthermore, the nested team formation mechanism helps to manage the complexity of communication within large agent teams. Assuming that the communication graph within each group chat is fully-connected, the number of edges in the graph represents the communication complexity. By decomposing a task into sub-tasks and allocating them to sub-group chats, the total number of edges can be reduced from $\frac{|\mathcal{C}_l|(|\mathcal{C}_l|-1)}{2}$ in the original group chat to $\sum_{g_{lj} \in h(g_l, s_{lj})} \frac{|\mathcal{C}_{lj}|(|\mathcal{C}_{lj}|-1)}{2}$ in the sub-group chats. This reduction in communication complexity leads to more efficient and focused collaboration among agents.


% \subsection{Autonomous Nested Team Formation}
% \label{sec:prototype-team-formation}

The primary motivation behind the autonomous nested team formation mechanism is to enable scalable and flexible task execution. Traditional multi-agent systems often struggle with static team compositions and limited scalability. By allowing agents to autonomously form nested teams, \framework can dynamically adjust to the complexity and scope of the task at hand, ensuring that agents with the appropriate skills and resources are engaged, leading to more efficient and effective problem-solving.

\paragraph{Mechanism Overview}
Autonomous nested team formation allows clients to dynamically form and expand teams to tackle complex tasks efficiently. This mechanism leverages the server's capabilities to discover and connect clients based on their skills and characteristics.

Let $\mathcal{C}$ denote the set of all clients in the system. For each client $c_i \in \mathcal{C}$, a description $d_i$ of the integrated agent's skills and capabilities is required upon registration. When a task $t$ is assigned to a client $c_i$, it enters the Team Formation Block with access to two tools: $\texttt{search\_client}$ and $\texttt{launch\_group\_chat}$. The $\texttt{search\_client}$ tool allows the client to discover other clients by querying the server's Agent Registry with a generated list of desired characteristics $\mathcal{L}_d = [l_1, l_2, \dots, l_k]$. The tool returns a subset of clients $\mathcal{C}_d \subseteq \mathcal{C}$ whose descriptions $d_j$ match the desired characteristics. The $\texttt{launch\_group\_chat}$ tool enables the client to initiate a group chat with the selected clients. The LLM in the client decides which tool to call, considering the retrieved information from the server, local information from the Agent Contact Block, and the task requirements.

\paragraph{Nested Team Formation}
\input{figs_code/nested-teamup}
In some cases, a single group may not be sufficient to complete a task. During discussions, agents may realize they need assistance from other agents with specific expertise. To address this, \framework supports nested team formation, allowing agents to initiate sub-group chats for sub-tasks. \cref{fig:nested-teamup} presents a simple example.

Let $t_l$ be a sub-task assigned to client $c_i$ in group chat $g$. If $c_i$ determines it cannot complete the task alone, it can search for appropriate clients for $t_l$ and initiate a new sub-group chat $g_{l}$, inviting a subset of other agents $\mathcal{C}_{l} \subseteq \mathcal{C}$ to collaborate on the sub-task. This process can continue recursively, forming a tree-like structure with the root representing the initial group chat and branches representing sub-group chats.

Furthermore, the nested team formation mechanism helps to manage the complexity of communication within large agent teams. Assuming that the communication graph within each group chat is fully connected, the number of edges in the graph represents the communication complexity. By decomposing a task into sub-tasks and allocating them to sub-group chats, the total number of edges can be reduced from $\frac{|g|(|g|-1)}{2}$ in the original group chat to $\sum_{l} \frac{|g_{l}|(|g_{l}|-1)}{2}$ in the sub-group chats, where $|g|$ and $|g_l|$ are the numbers of clients for task $t$ and $t_l$ respectively. This reduction in communication complexity leads to more efficient and focused collaboration among agents.



\subsection{Autonomous Conversation Flow Control}
\label{sec:prototype-conversation-flow}
Effective communication is crucial for successful collaboration among autonomous agents. Inspired by the Speech Act Theory~\citep{austin1975things, Searle_1969} and its application in conventional multi-agent systems~\citep{DBLP:conf/cikm/FininFMM94, DBLP:journals/expert/LabrouFP99}, we introduce an autonomous conversation flow control mechanism in \framework that enables agents to coordinate their communication and maintain a structured dialogue.

\paragraph{Sequential Speaking Mechanism}
Since the support for LLM interruption is still in its early stages, \framework adopts a sequential speaking mechanism, \textit{i.e.,} only one agent speaks at a time, preventing confusion and maintaining a clear order of communication. The simple and naive mechanism, when combined with the following dynamic features, leads to effective collaboration.

% \paragraph{Finite State Machine for Group Chat States}
% \input{figs_code/flow}
% We formalize the conversation flow as a finite state machine with five states: discussion, synchronous task assignment, asynchronous task assignment, pause \& trigger, and conclusion, as illustrated in~\cref{fig:flow}. These states represent different phases of the collaboration process and help agents navigate the conversation more efficiently. The states are closely related to the speech acts defined in the Speech Act Theory, such as assertives (discussion), directives (task assignment), commissives (pause \& trigger), and declarations (conclusion)~\citep{searle1976classification}.

% The \textit{discussion} state allows agents to engage in general dialogue, while the \textit{synchronous} and \textit{asynchronous task assignment} states enable task assignment with or without interrupting the ongoing discussion. The \textit{pause \& trigger} state introduces a mechanism for pausing the group chat and waiting for the completion of specified asynchronous tasks, and the \textit{conclusion} state marks the end of the collaboration.

% \paragraph{Autonomous State Transitions and Next Speaker Selection}
% State transitions in the conversation flow are decided by the LLM in the client, based on the current context and the progress of the collaboration. The LLM analyzes the messages exchanged and determines the most appropriate state to move the conversation forward. This decision-making process takes into account factors such as the completion of assigned tasks, the need for further discussion, and the overall goals of the collaboration.
% In addition to state transitions, the LLM also determines the next speaker in the conversation. The last speaker is responsible for designating the next agent to contribute to the dialogue, based on the current state and the expertise required. This selection process ensures that the most relevant agents are involved in the conversation at the appropriate times, promoting efficient information exchange and problem-solving.

\paragraph{Finite State Machine for Group Chat States}
\input{figs_code/flow}
We formalize the conversation flow as a finite state machine $M = (S, \Sigma, \delta, s_0, F)$, where:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=1.5em]
    \item $S = \{s_d, s_s, s_a, s_p, s_c\}$ is the set of states representing discussion, synchronous task assignment, asynchronous task assignment, pause \& trigger, and conclusion, respectively.
    \item $\Sigma$ is the input alphabet, which corresponds to the possible actions or events in the conversation flow.
    \item $\delta: S \times \Sigma \to S$ is the transition function that maps a state and an input to the next state.
    \item $s_0 = s_d$ is the initial state, representing the start of the conversation in the discussion phase.
    \item $F = \{s_c\}$ is the set of final states, containing only the conclusion state.
\end{itemize}

As illustrated in~\cref{fig:flow}, these states represent different phases of the collaboration process and help agents navigate the conversation more efficiently. The states are closely related to the speech acts defined in the Speech Act Theory, such as assertives (discussion), directives (task assignment), commissives (pause \& trigger), and declarations (conclusion)~\citep{searle1976classification}.

% Formally, let $\mathcal{A}$ be the set of all agents in the group chat, and let $a_i \in \mathcal{A}$ denote an individual agent. The current state of the conversation is represented by $s_t \in S$ at time step $t$. The transition function $\delta$ is defined as follows:
% \begin{align*}
%     \delta(s_d, \text{assign\_sync}) &= s_s \\
%     \delta(s_d, \text{assign\_async}) &= s_a \\
%     \delta(s_d, \text{pause\_trigger}) &= s_p \\
%     \delta(s_d, \text{conclude}) &= s_c \\
%     \delta(s_s, \text{complete\_sync}) &= s_d \\
%     \delta(s_a, \text{complete\_async}) &= s_d \\
%     \delta(s_p, \text{resume}) &= s_d
% \end{align*}

The \textit{discussion} state allows agents to engage in general dialogue, while the \textit{synchronous} and \textit{asynchronous task assignment} states enable task assignment with or without interrupting the ongoing discussion. The \textit{pause \& trigger} state introduces a mechanism for pausing the group chat and waiting for the completion of specified asynchronous tasks, and the \textit{conclusion} state marks the end of the collaboration.

\paragraph{Autonomous State Transitions and Next Speaker Selection}
State transitions in the conversation flow are decided by the LLM in the client, based on the current context and the progress of the collaboration. The LLM analyzes the messages exchanged and determines the most appropriate state to move the conversation forward. This decision-making process takes into account factors such as the completion of assigned tasks, the need for further discussion, and the overall goals of the collaboration.

Let $\mathcal{M}_t$ be the set of messages exchanged up to time step $t$, and let $f_{\text{LLM}}: \mathcal{M}_t \times S \to S \times \mathcal{A}$ be the decision function of the LLM that maps the conversation history and current state to the next state and the next speaker. The next state $s_{t+1}$ and the next speaker $a_{t+1}$ are determined as follows:
\begin{equation*}
    (s_{t+1}, a_{t+1}) = f_{\text{LLM}}(\mathcal{M}_t, s_t)
\end{equation*}

The selection of the next speaker $a_{t+1}$ ensures that the most relevant agents are involved in the conversation at the appropriate times, promoting efficient information exchange and problem-solving.

% \subsection{Comprehensive Message Protocol Design}
% \label{sec:prototype-message-protocol}

% The effectiveness of the autonomous nested team formation and conversation flow control mechanisms in \framework heavily relies on a well-designed message protocol. To enable seamless communication and collaboration among agents, we have developed a comprehensive agent message protocol that encapsulates all the necessary information required for the various mechanisms to function properly.

% \paragraph{Protocol Overview and Key Fields}
% The agent message protocol in \framework is designed to be extensible and flexible, allowing for the inclusion of a wide range of information that facilitates effective multi-agent collaboration. The structure of a message in \framework includes the following components:
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=2em]
%     \item \textbf{Header}: Contains essential information about the message, such as the sender's identity, the group chat's ID, the message type, and the next speaker. The header ensures that the message is correctly addressed and processed.
%     \item \textbf{Payload}: Carries the main content of the message, which varies depending on the message type. The payload can include team formation members (for team formation mechanism), triggers (for pause \& trigger mechanism), etc.
% \end{itemize}
% The detailed explanation and an example of the message protocol can be found in~\cref{sec:appendix-ioa-detail-message-protocol}. Both the client and server in \framework implement the message protocol to facilitate seamless communication. The client uses the protocol to encode and send messages to the server, the server routes them to the appropriate group chats, and the team members decode and act accordingly. This consistent implementation ensures that all agents can understand and respond to messages correctly, regardless of their specific roles or tasks.

% In summary, the comprehensive message protocol design in \framework is fundamental to the successful implementation of autonomous nested team formation and autonomous conversation flow control mechanisms. By providing a clear and consistent structure for message exchange, the protocol enables effective communication and coordination among agents, enhancing the overall performance of the multi-agent system.
\subsection{Comprehensive Message Protocol Design}
\label{sec:prototype-message-protocol}

The effectiveness of the autonomous nested team formation and conversation flow control mechanisms in \framework relies on a robust message protocol. This protocol enables seamless communication and collaboration among agents by encapsulating all necessary information required for various mechanisms to function properly.

\paragraph{Protocol Overview and Key Fields}
The agent message protocol in \framework is designed for extensibility and flexibility, facilitating effective multi-agent collaboration. The protocol consists of two main components: a header and a payload.

The header contains essential metadata about the message, ensuring correct addressing and processing by receiving agents. Key fields in the header include:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=1.5em]
    \item \texttt{sender}: The unique identifier of the agent sending the message.
    \item \texttt{group\_id}: The identifier of the group chat to which the message belongs.
\end{itemize}

The payload carries the main content of the message, varying by message type. It can include:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=1.5em]
    \item \texttt{message\_type}: Indicates the purpose of the message (e.g., discussion, task assignment, pause \& trigger).
    \item \texttt{next\_speaker}: The identifier(s) of the agent(s) expected to respond.
\end{itemize}

This structure contains other fields to support the diverse functionalities of \framework effectively. A detailed explanation and example of the message protocol can be found in~\cref{sec:appendix-ioa-detail-message-protocol}.

To ensure seamless communication and coordination, both the client and server components of \framework implement the message protocol. When a client sends a message, it encodes it according to the protocol and transmits it to the server. The server parses the message, extracts relevant information from the header, and routes it to the appropriate group chat based on the \texttt{group\_id}. Upon receiving a message, the client decodes it and processes it accordingly. This consistent implementation ensures that all agents can understand and respond to messages correctly, regardless of their roles or tasks, maintaining a coherent and efficient collaboration process.
